Relational Algorithms for k-means Clustering

This paper gives a k-means approximation algorithm that is efficient in the relational algorithms model. This is an algorithm that operates directly on a relational database without performing a join to convert it to a matrix whose rows represent the data points. The running time is potentially exponentially smaller than $N$, the number of data points to be clustered that the relational database represents. Few relational algorithms are known and this paper offers techniques for designing relational algorithms as well as characterizing their limitations. We show that given two data points as cluster centers, if we cluster points according to their closest centers, it is NP-Hard to approximate the number of points in the clusters on a general relational input. This is trivial for conventional data inputs and this result exemplifies that standard algorithmic techniques may not be directly applied when designing an efficient relational algorithm. This paper then introduces a new method that leverages rejection sampling and the $k$-means++ algorithm to construct an O(1)-approximate k-means solution.

==> Algo_Guiding_Rule.tex <==
\section{Guiding Rules of Algorithm Design}



Suppose we are given data set $S$. The \emph{adaptive k-means++ clustering} algorithm proposed in \cite{aggarwal2009adaptive} follows this routine:

\begin{itemize}
    \item Sample $\kp = O(k)$ centers $\cC = \{ C_1, \ldots, C_\kp \}$. according to the $k$-means++ sampling rule.
    \item Calculate the number of points in $\as_S(C_i)$ for all centers $C_i$, denote the set of weights by $\cW = \{w_1, \ldots, w_\kp \}$.
    \item Weight every center $C_i$ by $w_i$, and solve the weighted $k$-means problem on the weighted input $(\cC, \cW)$.
\end{itemize}

We cite the following theorem from \cite{aggarwal2009adaptive} (Theorem 1 in the paper), which says the algorithm gives $O(1)$-approximation for optimal $k$-means objective value with constant probability.

\begin{theorem}[\cite{aggarwal2009adaptive}]
\label{thm:adaptive_approx}
Denote the optimal $k$-means centers by $\cC_\opt$, and let $\phi_\opt = \phi_S(\cC_\opt))$ be the optimal $k$-means objective value. If $\kp = \lfloor 16(k + \sqrt{k}) \rfloor$. Let $\cC \subseteq S$ be the set of centers sampled in the above algorithm, then, $\phi_S(\cC) \leq 20 \phi_\opt$ with probability at least $0.03$. \alireza{Should we use the weights somewhere?}
\end{theorem}

\yuyan{we need to figure out what to put here?}

\begin{algorithm}
    \caption{In-database adaptive $k$-means++}\label{alg:main_algo}
    \begin{algorithmic}[1]
        \Procedure{AdaptiveKMeans++}{$S, k, \eps$}
            \State $\kp \gets \lfloor 16(k+\sqrt{k}) \rfloor$.
            \State $\cC \gets \emptyset$.
            \For{$i = 1,\ldots, \kp$}
                \State $C_i \gets \text{Kmeans++Sample}(S,\cC)$
                \State $\cC \gets \cC \cup \{ C_i\}$ 
            \EndFor
        \State $\cW \gets \{\text{EstimateWeights}(S, \cC, \eps)\}$
        \State Return the optimal centers for weighted $k$-means on $(\cC, \cW)$.
        \EndProcedure
    \end{algorithmic}
\end{algorithm}
